An algebraic formulation of the graph reconstruction conjecture

The graph reconstruction conjecture asserts that every finite simple graph on at least three vertices can be reconstructed up to isomorphism from its deck - the collection of its vertex-deleted subgraphs. Kocay's Lemma is an important tool in graph reconstruction. Roughly speaking, given the deck of a graph $G$ and any finite sequence of graphs, it gives a linear constraint that every reconstruction of $G$ must satisfy. Let $\psi(n)$ be the number of distinct (mutually non-isomorphic) graphs on $n$ vertices, and let $d(n)$ be the number of distinct decks that can be constructed from these graphs. Then the difference $\psi(n) - d(n)$ measures how many graphs cannot be reconstructed from their decks. In particular, the graph reconstruction conjecture is true for $n$-vertex graphs if and only if $\psi(n) = d(n)$. We give a framework based on Kocay's lemma to study this discrepancy. We prove that if $M$ is a matrix of covering numbers of graphs by sequences of graphs, then $d(n) \geq \mathsf{rank}_\mathbb{R}(M)$. In particular, all $n$-vertex graphs are reconstructible if one such matrix has rank $\psi(n)$. To complement this result, we prove that it is possible to choose a family of sequences of graphs such that the corresponding matrix $M$ of covering numbers satisfies $d(n) = \mathsf{rank}_\mathbb{R}(M)$.

==> conclusion.tex <==
\section{Discussion}

In this paper we have described an algebraic formulation of the graph
reconstruction conjecture. Our results show that if this conjecture is
true then, at least in principle, it may be proven using equations
obtained from Kocay's lemma, and we believe that further investigation
of this approach may be fruitful. For example, it will be interesting to
prove that trees are reconstructible using the approach of this
paper. On the other hand, existence of non-reconstructible directed
graphs (particularly tournaments) and hypergraphs may also be proved by
an algebraic approach based on Kocay's lemma.

The approach may also be useful to study questions about
\emph{legitimate decks}: a collection of $n$-vertex graphs, each of
which has $n-1$ vertices, is called a \emph{legitimate deck} if it is
the collection of vertex-deleted subgraphs of an $n$-vertex
graph. Harary \cite{harary-1969} asked for a characterisation of
legitimate decks.

Now suppose that $\mcf$ is a sequence of $n$ graphs, each on $(n-1)$
vertices, that is not a legitimate deck. In the proof of Theorem
\ref{t:converse}, we observe that a sequence equivalent to $\mcf$ does
not appear in the recurrence relations for non-overlapping covering
numbers of other sequences. Therefore, deleting the row corresponding to
$\mcf$ (or corresponding to a sequence equivalent to it) from $M$ does
not change the rank of $M$. Can we extend such arguments further to
completely characterise legitimate decks?

% Several interesting results in reconstruction theory have been obtained
% by algebraic methods, and we believe that further investigation of this
% approach may be fruitful. In particular, it would be interesting to see
% a new proof that trees are reconstructible derived directly from Theorem
% \ref{t:main}. \query{Comment}{I don't understand the first line. Maybe
%   this paragraph needs to be rephrased.}


==> legitimate.tex <==
\section{Comments on the legitimate deck problem}
The approach may also be useful to study questions about legitimate
decks. A collection of $n$ graphs, each with $(n-1)$ vertices, is
considered \emph{legitimate} if it is the deck of some graph. The
\emph{legitimate deck problem}, posed by Harary \cite{harary-1969}, asks
for a characterisation of legitimate decks. It would be interesting to
determine how the rank of the matrix $M$ defined in Theorem
\ref{t:converse} changes if either some of the legitimate or the
illegitimate decks are ignored while setting up $M$.

Suppose that $\mcf$ is a sequence of $n$ graphs, each on $(n-1)$
vertices, that is not a legitimate deck. In the proof of Theorem
\ref{t:converse}, we observe that a sequence equivalent to $\mcf$ does
not appear in the recurrence relations for non-overlapping covering
numbers of other sequences. Therefore, deleting the row corresponding
to $\mcf$ (or corresponding to a sequence equivalent to it) from $M$
does not change the rank of $M$. What if the row corresponding to a
legitimate deck is removed from $M$?  We have to formulate this
question a bit carefully, since the reconstruction class of a graph
$G$ may be determined uniquely by a subset of its deck, in which case
deleting a sequence of the deck of $G$ may not change the rank of
$M$. In the following, we try to make the question a little more
precise.

Let $\mathfrak{F}$ be the family of all mutually inequivalent
sequences of length $k$ of $(n-1)$-vertex graphs, where $2 \leq k \leq
n$. Here the term \emph{inequivalent} is used as defined in the proof
of Theorem~\ref{t:converse}. We say that a sequence $\mcf \coloneqq
(F_1,F_2,\dots, F_k) \in \mathfrak{F}$ is legitimate if there is a
graph $G$ and a one-one map $f:\{1,2,\dots,k\}\rightarrow V(G)$ such
that $F_i \cong G-f(i)$ for all $i \in \{1,2,\dots,k\}$; in this case,
we say that $\mcf$ is a \emph{sub-deck} of $G$. Otherwise, we say
$\mcf$ is illegitimate. We say that a legitimate sequence $\mcf$ is
minimal if it determines a unique reconstruction class, but none of
its proper subsequences determines a unique reconstruction class; in
other words, if $\mcf$ is a sub-deck of graphs $G$ and $H$ then $G$
and $H$ belong to the same reconstruction class, but for every proper
subsequence $\mcf^\prime$ of $\mcf$, there exist graphs $G$ and $H$
from different reconstruction classes that have $\mcf^\prime$ as a
sub-deck. Next we define a partial order $\leq$ on $\mathfrak{F}$:
given $\mcf_1 \coloneqq (F_1,F_2,\dots,F_k)$ and $\mcf_2 \coloneqq
(F_1^\prime,F_2^\prime,\dots,F_\ell^\prime)$, we say that $\mcf_1 \leq
\mcf_2$ if there is a one-one map $f:\{1,2,\dots,k\}\rightarrow
\{1,2,\dots,l\}$ such that $F_i \cong F_{f(i)}^\prime$. Now if a
sequence $\mcf \in \mathfrak{F}$ is illegitimate, then all sequences
above $\mcf$ are illegitimate.

\begin{problem}
 Is there a characterisation of legitimate sequences and minimal
 legitimate sequences in terms of the effect of the removal of the
 corresponding rows from $M$? Suppose that $\{\mcf_i \mid i =
 1,2,\dots, k\}$ is a minimal family of sequences such that deleting
 the rows of $M$ corresponding to sequences in the upper set of
 $\{\mcf_i \mid i = 1,2,\dots, k\}$ decreases the rank of $M$ by
 exactly 1, then are $\mcf_i, i = 1,2,\dots, k$ minimal legitimate
 sequences of a single reconstruction class?
\end{problem}

